Double Critic Deep Reinforcement Learning for Mapless 3D Navigation of Unmanned Aerial Vehicles

This paper presents a novel deep reinforcement learning-based system for 3D mapless navigation for Unmanned Aerial Vehicles (UAVs). Instead of using a image-based sensing approach, we propose a simple learning system that uses only a few sparse range data from a distance sensor to train a learning agent. We based our approaches on two state-of-art double critic Deep-RL models: Twin Delayed Deep Deterministic Policy Gradient (TD3) and Soft Actor-Critic (SAC). We show that our two approaches manage to outperform an approach based on the Deep Deterministic Policy Gradient (DDPG) technique and the BUG2 algorithm. Also, our new Deep-RL structure based on Recurrent Neural Networks (RNNs) outperforms the current structure used to perform mapless navigation of mobile robots. Overall, we conclude that Deep-RL approaches based on double critic with Recurrent Neural Networks (RNNs) are better suited to perform mapless navigation and obstacle avoidance of UAVs.

==> sections/4_theorethical.tex <==
\section{Theoretical Background}
\label{theoretical}

Deep-RL is actively used to perform tasks in the discrete action spaces. It was used to achieve a performance similar to a human when playing the Atari video games \cite{mnih2013playing}. A different kind of Deep-RL algorithm that can perform in the continuous actions space must be used to address navigation related problems for mobile robots\cite{lillicrap2015continuous}. Here are the state-of-art techniques for this kind of problem that was used to implement our approaches

\subsection{Twin Delayed Deep Deterministic Policy Gradient}

The methods of value-based reinforcement learning such as DQN \cite{mnih2013playing} and actor-critic setting as in the work of Lillicrap \emph{et al.} \cite{lillicrap2015continuous} are known to lead to value estimates and suboptimal policies. This overestimation bias is a property of Q-Learning in which the insertion of noisy value estimate causes a consistent overestimation \cite{thrun1993issues}.

The Twin Delayed Deep Deterministic Policy Gradient (TD3) \cite{fujimoto2018addressing} is an actor-critic algorithm that considers the interaction between function approximation error both policy and value updates.
This algorithm employed two neural networks: one that represents the actor-network and it is responsible to learn the policy, and the other that represents the critic network that approximates the Q-function.
The two neural networks are in charge of the action prediction for the current observation state and they generate a temporal-difference error signal for each time step.
In the critic, we have the Double Q-learning method \cite{hasselt2010double} in which the update is freed from the value function by maintaining two separates estimates $Q_1$ and $Q_2$.
This addresses the problem of overestimation bias induced by the use of only one estimation of the value of state $Q$.

Target networks are a well-known tool to achieve stability in deep reinforcement learning \cite{mnih2013playing}.
The TD3 demonstrates that policy updates on high-error states cause divergent behavior.
With this, it was formulated in such a way that the policy network, also known as actor network, should be updated at a lower frequency than the value network, to first minimize error before introducing a policy update. 
Therefore, the policy is delayed until the error of value is minimal as possible. 
The update of the policy and target networks are made after a fixed number of updates of the critic network.
Nonetheless, to ensure that the temporal difference remains small between the policy network $\theta$ and target network $\theta'$, which can regulate the learning and improvement stability, it is updated the target networks slowly using Poliak Averaging \cite{polyak1992acceleration}:

\begin{equation}
    \theta' \leftarrow \tau\theta + (1-\tau)\theta'
\end{equation}
where $\tau$ is hyperparameter between 0 and 1 for controlling of the learning process of the target network, and $\theta$ represents the weights of the main network, as well as, the $\theta'$ represents the weights of target network.

A concern with deterministic policies is that they can overfit to narrow peaks in the value estimate, being one of the great challenges of learning in continuous and discrete action space.
To overcome this problem, it is added a small amount of random noise to the target action. 
This makes it harder for the policy to exploit Q-function errors and to explore new states by the agent.

\subsection{Soft Actor-Critic}

The Soft Actor Critic (SAC) algorithm is also a actor-critic method. Differently than TD3, SAC learns the policies in the continuous action space by using approximation functions\cite{haarnoja2018soft}. 
The algorithm makes use of a neural network for the actor-network, the value network and other for the critic network. 
% These three networks compute the action prediction for the current state and generate a temporal-difference error signal for each time step.

Instead of only seeking to maximize the rewards of the system, SAC seeks to also maximize the entropy of the policy.
The entropy refers to how unpredictable a variable can be. 
So, if a random variable always takes a single value then it has zero entropy because it is not unpredictable at all. 
The high entropy in the policy explicitly encourages exploration of the agent because it assigns equal probability to actions that have the same or nearly equal Q-value and also to ensure that it does not collapse into repeatedly selecting a particular action that could exploit some inconsistency in the approximated Q function.

In general, for training and evaluating the policy function output from the actor network, and the value function and the Q-function output from from the critic network, it is recommended to make use of a replay memory. This technique saves the experiences given by the agent during the training session \cite{schaul2015prioritized}.
The states, actions, rewards and new states that an agent experimented in the previous episodes are saved into a memory buffer, being marked as an experience.
When a minimal number of experiences are stored into memory, then these experiences, which occurred in previous episodes, are randomly sampled for the learning of the algorithm.
These TD3 and SAC techniques with replay memory can stop the temporal correlations between different episodes in the training phase.
Even though with short memories, it is noticeable a significant increase in the performance of the off-policy Deep-RL algorithms.
Regardless of the boost in the capabilities in application with Deep-RL, the use of replay memories can affect the learning time of an agent by making it slower but more reliable.
Despite the use of replay memories, the Q-learning algorithms make use of target networks as the TD3 makes use.



